Consistency and Accuracy of CelebA Attribute Values

We report the first systematic analysis of the experimental foundations of facial attribute classification. Two annotators independently assigning attribute values shows that only 12 of 40 common attributes are assigned values with >= 95% consistency, and three (high cheekbones, pointed nose, oval face) have essentially random consistency. Of 5,068 duplicate face appearances in CelebA, attributes have contradicting values on from 10 to 860 of the 5,068 duplicates. Manual audit of a subset of CelebA estimates error rates as high as 40% for (no beard=false), even though the labeling consistency experiment indicates that no beard could be assigned with >= 95% consistency. Selecting the mouth slightly open (MSO) for deeper analysis, we estimate the error rate for (MSO=true) at about 20% and (MSO=false) at about 2%. A corrected version of the MSO attribute values enables learning a model that achieves higher accuracy than previously reported for MSO. Corrected values for CelebA MSO are available at https://github.com/HaiyuWu/CelebAMSO.

==> supplementary_marterial_figure_text_files/edge_images.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/010603.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/007370.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/024935.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/033855.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/051909.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/054744.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/058142.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/060818.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/066111.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/070090.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/072351.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/085981.jpg}
                    
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/088673.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/010874.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/091223.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/035859.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/095442.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/041852.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/105927.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/107047.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/110704.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/114312.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/114370.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/140655.jpg}
                    
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/140926.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/049825.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/088545.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/110722.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/145264.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/148806.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/150988.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/151095.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/156961.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/160322.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/161960.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/167839.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/173206.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/187401.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/190465.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/190595.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/180201.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/edge_images/017538.jpg}
                    
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of the edge cases of MSO attribute.}
\label{fig:edge-images}
\end{figure}

==> supplementary_marterial_figure_text_files/gradcams.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202297.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202297.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202305.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202305.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202309.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202309.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202310.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202310.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202318.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202318.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202324.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202324.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202330.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202330.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202331.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202331.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_202333.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/0/MOON_clean__202333.jpg}
                \end{subfigure}
            \end{subfigure}
        \caption{Samples of Score-CAM when MOON-original and MOON-ours predict MSO=False}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202433.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202433.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202469.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202469.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202476.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202476.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202483.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202483.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202486.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202486.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202489.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202489.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202492.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202492.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202498.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202498.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_202505.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/gradcams/1/MOON_clean__202505.jpg}
                \end{subfigure}
            \end{subfigure}
        \caption{Samples of Score-CAM when MOON-original and MOON-ours predict MSO=True}
        \end{subfigure}
    \end{subfigure}
   \caption{Examples of Score-CAMs. The images are shown in pairs. For each image pair, the image on the left is from the model created using original dataset, the image on the right is from the model created using our dataset.}
\label{fig:gradcams}
\end{figure}



==> supplementary_marterial_figure_text_files/inconsistent_definitions.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/003867.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/004367.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/005163.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/006879.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/007007.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/012361.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/015266.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/016276.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/021535.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/024546.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/027277.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/bald/029505.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of bald=true in original dataset}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/000252.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/028003.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/029674.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/032748.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/048306.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/064799.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/071344.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/079256.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/088536.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/095443.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/097621.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/gray_hair/112537.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of gray\_hair=true in original dataset}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/001039.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/001157.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/006244.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/007466.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/007525.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/007644.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/011010.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/011808.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/016133.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/017514.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/018292.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/inconsistent_definitions/mso/018866.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of MSO=false in original dataset.}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Error samples that are caused by the inconsistent definition.}
\label{fig:inconsistent-definition}
\end{figure}

==> supplementary_marterial_figure_text_files/information_lost.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/001500.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/001500.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/007174.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/007174.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/008760.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/008760.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/009927.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/009927.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/010976.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/010976.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/013791.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/013791.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/015535.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/015535.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/016404.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/016404.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/after-alignment/017638.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necklace/before-alignment/017638.jpg}
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of Wearing\_Necklace=true in original dataset}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/013994.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/013994.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/013999.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/013999.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/018259.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/018259.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/035125.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/035125.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/037092.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/037092.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/047752.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/047752.jpg}
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/059474.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/059474.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/059963.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/059963.jpg}
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{0.32\linewidth}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/after-alignment/068721.jpg}
                \end{subfigure}
                \begin{subfigure}[b]{0.49\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_lost/Wearing_Necktie/before-alignment/068721.jpg}
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of Wearing\_Necktie=true in original dataset}
        \end{subfigure}
    \end{subfigure}
   \caption{Error samples that are caused by the less information. The images are shown in pairs. For each image pair, the aligned image is on the left, the original image is on the right.}
\label{fig:information-lost}
\end{figure}



==> supplementary_marterial_figure_text_files/information_not_visible.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
    \captionsetup[subfigure]{labelformat=empty}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/001401.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/001469.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/002944.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/004010.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/004104.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/004165.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/004252.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/004332.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/004689.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/005018.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/014842.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/015507.jpg}
                    
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/015549.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/016303.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/017065.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/017069.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/017246.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/018979.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/020918.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/021496.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/021781.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/021888.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/022398.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/022750.jpg}
                    
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/023340.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/025948.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/026454.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/026742.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/026822.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/027468.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/028532.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/031162.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/032833.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/034411.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/035255.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/036297.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/038276.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/039697.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/061258.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/112069.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/112324.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/information_not_visible/117500.jpg}
                    
                \end{subfigure}
            \end{subfigure}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of the third annotation option: information not visible.}
\label{fig:imformation-not-visible}
\end{figure}

==> supplementary_marterial_figure_text_files/short_length_of_facial_hair.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/000408.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/001290.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/007345.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/010632.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/017553.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/043387.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/018661.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/024795.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/037061.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/042800.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/043083.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/goatee/048231.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of goatee=true in original dataset}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/002925.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/003314.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/004664.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/005397.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/006914.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/029607.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/011037.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/016474.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/017779.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/019822.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/026239.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/short_length_of_facial_hair/no_beard/030411.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Error samples of no\_Beard=false in original dataset}
        \end{subfigure}
    \end{subfigure}
   \caption{Error samples that are caused by the short length of facial hair.}
\label{fig:short-length-of-facial-hair}
\end{figure}

==> supplementary_marterial_figure_text_files/unusable_images.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{1\linewidth}
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/011793.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/016530.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/019205.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/024184.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/026135.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/031125.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/039459.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/041897.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/048286.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/080480.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/092651.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/corrupted_images/102061.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Examples of corrupted images in the original dataset.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/006531.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/009111.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/019377.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/022629.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/027964.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/039816.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/040604.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/042291.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/044200.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/049114.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/050199.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/face_paint/058362.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Examples of heavy-face-painting or face-mask images in the original dataset.}
        \end{subfigure}
        
        \begin{subfigure}[b]{1\linewidth}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/030452.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/030468.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/036696.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/037586.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/038651.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/049079.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \begin{subfigure}[b]{1\linewidth}
            \centering
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/050658.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/053101.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/066700.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/067788.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/068337.jpg}
                    
                \end{subfigure}
                \begin{subfigure}[b]{0.15\linewidth}
                    \includegraphics[width=\linewidth]{supplementary_marterial_figures/unusable_images/two_faces/068992.jpg}
                    
                \end{subfigure}
            \end{subfigure}
            \caption{Examples of two-faces images in the original dataset.}
        \end{subfigure}
        
    \end{subfigure}
   \caption{Examples of the part of the unusable images. The main issue of the unusable images is no faithful facial attributes, or more than one faces in the image.}
\label{fig:unusable-images}
\end{figure}
